Towards Understanding and Avoiding Limitations of Convolutions on Graphs

While message-passing neural networks (MPNNs) have shown promising results, their real-world impact remains limited. Although various limitations have been identified, their theoretical foundations remain poorly understood, leading to fragmented research efforts. In this thesis, we provide an in-depth theoretical analysis and identify several key properties limiting the performance of MPNNs. Building on these findings, we propose several frameworks that address these shortcomings. We identify two properties exhibited by many MPNNs: shared component amplification (SCA), where each message-passing iteration amplifies the same components across all feature channels, and component dominance (CD), where a single component gets increasingly amplified as more message-passing steps are applied. These properties lead to the observable phenomenon of rank collapse of node representations, which generalizes the established over-smoothing phenomenon. By generalizing and decomposing over-smoothing, we enable a deeper understanding of MPNNs, more targeted solutions, and more precise communication within the field. To avoid SCA, we show that utilizing multiple computational graphs or edge relations is necessary. Our multi-relational split (MRS) framework transforms any existing MPNN into one that leverages multiple edge relations. Additionally, we introduce the spectral graph convolution for multiple feature channels (MIMO-GC), which naturally uses multiple computational graphs. A localized variant, LMGC, approximates the MIMO-GC while inheriting its beneficial properties. To address CD, we demonstrate a close connection between MPNNs and the PageRank algorithm. Based on personalized PageRank, we propose a variant of MPNNs that allows for infinitely many message-passing iterations, while preserving initial node features. Collectively, these results deepen the theoretical understanding of MPNNs.

==> chapter4/related_work.tex <==
\section{Related Work}
We now describe previous works related to various parts of the MIMO-GC and the LMGC.
\paragraph{Derivation of MPNNs}


% Multi-channel learning in MPNNs
 \paragraph{}






% Similarities of the LMGC with other methods
\paragraph{Approaches Related to the LMGC}
%expressivity
The LMGC is closely related to several existing methods. As described in \cref{ex:gat}, multi-head attention-based methods like GAT~\parencite{veličković2018graph} and GATv2~\parencite{brody2022how} are LMGCs with constraints on the attention scores by applying the softmax activation. By lifting this constraint, LMGCs can be injective on multisets (\cref{prop:injectivity}). Several other methods have been proposed to replace the softmax activation. The FAGCN~\parencite{bo2021beyond} instead applies the tanh activation function to amplify high-frequencies or low-frequencies. Similarly, the GGCN~\parencite{yan2022two} allows learning of signed edge weights.  %avoid over-smoothing
Other studies considered replacing the softmax activation function within transformers and self-attention modules. \textcite{wortsman2023replacing} apply the ReLU activation in vision transformers. \textcite{saratchandran2024rethinking} found empirical success using polynomial activation functions for self-attention. 
However, as self-attention typically considers a fully connected graph, these works did not study distinguishing structural differences. 
Contrarily, \cref{prop:injectivity} shows that differences in the number of neighbors can be distinguished without the softmax activation. 


%multi-head approaches, learnable edge weights (GAT, GATv2, velickovic, replacing softmax,..., tanh)
%Spectral Graph Convolutions
%\parencite{levie2021transfer} transferability of spectral graph convolutions
%\parencite{koke2023limitless} transferability of spectral graüh convolitposns
%\parencite{koke2024holonets} extended spectral convolutions to directed graphs.
%\parencite{he2021bernnet} basis in which the filter is learned
%\parencite{levis2019cayleynets}
%\parencite{wang2022how}

%\section{Related Work}



==> chapter5/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
%Summary
In this chapter, we considered the challenge of ensuring localization of representations after applying message-passing iterations. As this is caused by the dominance of the first eigenvector, which is similarly the case in the PageRank algorithm, we considered solutions proposed for the PageRank algorithm. This is personalized PageRank which adds a chance to teleport back to the initial state during the random walk. While previous work similarly tried to do this, it was not achieved with unconstrained feature transformations, they were either constrained in their spectrum, or they were omitted entirely. By following the sequence of the exponential function, we allow for unconstrained feature transformations while being able to prove convergence to a unique solution.
%Fits into greater context
This concept also allows arbitrary message-passing algorithms, even multiple aggregation matrices or computational graphs.
Our findings allow a different approach to the commonly predefined number of iterations or layers. The depth can be learned adaptively by model removing the need to carefully tune this parameter.
Future research can incorporate these results for better performance and combine it with other techniques such as better message-passing than the GCN.
The field can now focus on other things.
%Limitations
While this solves the issue of losing locality, the combination with other techniques remains open. While we have shown much potential for various benchmark dataset, it remain open for which application ensuring locality while allowing infinite-depth is particularly desirable.

%We introduced PPRGNN, a reformulation of MPNNs based on personalized PageRank that assures localization and prevents over-smoothing of node features even when using infinitely many layers.
%message passing neural network based on the idea of personalized PageRank that also utilizes learnable weights. 
%Theoretically based on the personalized version of PageRank which allows teleporting back to the initial state, we adopt this idea for MPNNs, specifically for the basic type GCNs~\parencitep{kipf2016semi}. Starting from the classic algorithm, we follow intuitive steps to introduce learnable parameters and still converge to a limit distribution.
%Compared to previous infinite-depth GNNs, our approach has a higher modeling capacity as we do not place any constraints.
%Our empirical evaluation on tasks for graph classification, and inductive and transductive node classification 
%confirm our theoretical base. Against regular GCNs that have no way to teleport back to the initial state, we find large improvements across all datasets. We even outperform other comparable approaches, including previous infinite-depth models, across almost all datasets by decent margins.
%Despite the theoretical infinite-depth, we introduced a path for efficient optimization, running linearly in the number of layers and only using constant memory. Our formulation allows controlling the convergence rate, leading to considerable improvements in experimental execution time compared to IGNN, a previous infinite-depth model. 
%While we show that our formulation allows infinitely many layers, even fixed sized models should benefit from adopting our idea. Our approach is directly applicable to other types of MPNNs, for which our proofs of convergence should hold.


==> contributions_figure.tex <==
\begin{tikzpicture}[x=\textwidth/4, y=\textwidth/4]
\definecolor{vibrantblue}{HTML}{a6cee3} % Boxes
\definecolor{vibrantgreen}{HTML}{b2df8a} %Circles
\definecolor{vibrantpink}{HTML}{fb9a99} %Contributions
\definecolor{vibrantorange}{HTML}{fdbf6f} %MIMO
\definecolor{vibrantpurple}{HTML}{cab2d6} %SISO
\definecolor{vibrantsand}{HTML}{ffff99} %Kreise
%\definecolor{vibrantmagenta}{HTML}{EE3377}
%\definecolor{vibrantgray}{HTML}{BBBBBB}
\usetikzlibrary{shapes}
\pgfdeclarelayer{background}
\pgfsetlayers{background,main}
\tikzset{
dot/.style = {circle, minimum size=#1,
              inner sep=0pt, outer sep=0pt, draw=black},
dot/.default =13pt  % size of the circle diameter 
}
    % Define the colors and styles
    \tikzstyle{box} = [draw, draw=vibrantblue, thick,rounded corners,line width=1.8pt]

    \def\yconv{1.6}
    \def\ysiso{-0.2}
    \def\yover{0.7}
    \def\ymethods{-1.1}
    \def\xshift{1.0}
    
    % Polynomials
    \def\xpoly{0.0}
    \node[rectangle,draw=vibrantblue,minimum height=3cm,minimum width=5.2cm, rounded corners, line width=1mm] at (\xpoly,\yconv) (chapter2) {};
    %\draw[box] (\xpoly -0.65, \yconv-0.4) rectangle (\xpoly + 0.65, \yconv+0.4);  % Center vertical box
    %\node at (\xpoly, \yconv+0.4) {Polynomials};
    
    \node[fill=vibrantsand,minimum width=3.5cm,minimum height=2cm,draw,ellipse] (conv) at (\xpoly,\yconv) {};
    \node[scale=0.7,align=center]  at (\xpoly, \yconv) {Graphs \& \\Graph Convolution \& \\ MPNNs}; 
    \node[scale=1.0] at (\xpoly-0.4, \yconv + 0.3) {Chapter 2};
    \node[scale=1.0,align=center] at (\xpoly-\xshift-1.1, \yconv) {Fundamentals};

    
    % Draw horizontal boxes
    \node[rectangle,draw=vibrantpurple,minimum height=6.2cm,minimum width=13cm, rounded corners, line width=1mm] at (\xpoly,\ysiso+0.45) (chapter3) {}; % Top horizontal box
    \node[scale=1.0] at (\xpoly-\xshift-0.4, \yover+0.22) {Chapter 3}; % Bottom-left horizontal + vertical
    \node[scale=1.0,align=center] at (\xpoly-\xshift-1.1, \ysiso+0.45) {Understanding \\ Over-Smoothing};
    
    %\node at (-1.20, \ysiso) {}; 
    % SC Polynomials
    \node[fill=vibrantsand,minimum width=3.5cm,minimum height=2cm,draw,ellipse] (over-smoothing) at (\xpoly,\yover) {};
    \node[scale=0.7,align=center]  at (\xpoly, \yover) {Over-Smoothing}; 
    %\node[scale=0.7] at (\xpoly, \ysiso - 0.1) {(\autoref{eq:siso_poly})}; 

    % MC Polynomials
    \node[fill=vibrantsand,minimum width=3.5cm,minimum height=2cm,draw,ellipse] (rankcollapse) at (\xpoly,\ysiso) {};
    \node[scale=0.7] at (\xpoly, \ysiso) {Rank Collapse};   
    
    \node[fill=vibrantsand,minimum width=3.5cm,minimum height=2cm,draw,ellipse] (mcpoly) at (\xpoly-\xshift,\ysiso) {};
    \node[scale=0.7] at (\xpoly-\xshift, \ysiso) {Filter Uniformity};   
    %\node[scale=0.7] at (\xpoly-\xshift, \ymimo - 0.1) {(\autoref{eq:mimo_poly})}; 

    % MC Polynomials
    \node[fill=vibrantsand,minimum width=3.5cm,minimum height=2cm,draw,ellipse] (dominance) at (\xpoly+\xshift,\ysiso) {};
    \node[scale=0.7] at (\xpoly+\xshift, \ysiso) {Signal Dominance};   
    %\node[scale=0.7] at (\xpoly+\xshift, \ymimo - 0.1) {(\autoref{eq:mimo_poly})}; 


    \node[rectangle,draw=vibrantpurple,minimum height=3cm,minimum width=5.2cm, rounded corners, line width=1mm] at (\xpoly-\xshift,\ymethods) (chapter4) {};
    %\draw[box,draw=vibrantpurple] (\xpoly-\xshift -0.65, \ymethods-0.4) rectangle (\xpoly-\xshift + 0.65, \ymethods+0.4);  % Center vertical box
    \node[scale=1.0] at (\xpoly-\xshift-0.4, \ymethods + 0.3) {Chapter 4};

    \node[rectangle,draw=vibrantpurple,minimum height=3cm,minimum width=5.2cm, rounded corners, line width=1mm] at (\xpoly+\xshift,\ymethods) (chapter5) {};
    %\draw[box,draw=vibrantpurple] (\xpoly+\xshift -0.65, \ymethods-0.4) rectangle (\xpoly+\xshift + 0.65, \ymethods+0.4);  % Center vertical box
    \node[scale=1.0] at (\xpoly+\xshift+0.4, \ymethods + 0.3) {Chapter 5};


    \node[scale=1.0,align=center] at (\xpoly-\xshift-1.1, \ymethods) {Solutions};

    % MC Polynomials
    \node[fill=vibrantsand,minimum width=3.5cm,minimum height=2cm,draw,ellipse] (lmgc) at (\xpoly-\xshift,\ymethods) {};
    \node[scale=0.7,align=center] at (\xpoly-\xshift, \ymethods) {Multiple \\Computational Graphs};   
    %\node[scale=0.7] at (\xpoly-\xshift, \ymethods - 0.1) {(\autoref{eq:mimo_poly})}; 

    % MC Polynomials
    \node[fill=vibrantsand,minimum width=3.5cm,minimum height=2cm,draw,ellipse] (pprgnn) at (\xpoly+\xshift,\ymethods) {};
    \node[scale=0.7,align=center] at (\xpoly+\xshift, \ymethods) {Restarting \\Message-Passing};   
    %\node[scale=0.7] at (\xpoly+\xshift, \ymethods - 0.1) {(\autoref{eq:mimo_poly})}; 

    %\draw[->,line width=1.2pt] (conv) to node[sloped,above,color=black,scale=0.7,rotate=90] {} (over-smoothing);
    \draw[->,line width=1.2pt] (over-smoothing) to node[sloped,above,color=black,scale=0.7,rotate=90] {} (mcpoly);
    %\draw[->] (scmpnn) -- (mcmpnn)
    \draw[->,line width=1.2pt] (over-smoothing) to node[sloped,above,color=black,scale=0.7,rotate=90] {} (dominance);
    \draw[->,line width=1.2pt] (over-smoothing) to node[sloped,above,color=black,scale=0.7,rotate=90] {} (rankcollapse);
    \draw[->,line width=1.2pt] (conv) to node[sloped,above,color=black,scale=0.7,rotate=90] {} (chapter3);
    \draw[->,line width=1.2pt] (mcpoly) to node[sloped,above,color=black,scale=0.7,rotate=90] {} (chapter4);
    \draw[->,line width=1.2pt] (rankcollapse) to node[sloped,above,color=black,scale=0.7,rotate=90] {} (chapter4);
    \draw[->,line width=1.2pt] (dominance) to node[sloped,above,color=black,scale=0.7,rotate=90] {} (chapter5);
    \draw[->,line width=1.2pt] (rankcollapse) to node[sloped,above,color=black,scale=0.7,rotate=90] {} (chapter5);    
    
\end{tikzpicture}
